On the Cost-Optimality Trade-off for Service Function Chain Reconfiguration

Optimal placement of Virtual Network Functions (VNFs) in virtualized data centers enhances the overall performance of Service Function Chains (SFCs) and decreases the operational costs for mobile network operators. Maintaining an optimal placement of VNFs under changing load requires a dynamic reconfiguration that includes adding or removing VNF instances, changing the resource allocation of VNFs, and re-routing corresponding service flows. However, such reconfiguration may lead to notable service disruptions and impose additional overhead on the VNF infrastructure, especially when reconfiguration entails state or VNF migration. On the other hand, not changing the existing placement may lead to high operational costs. In this paper, we investigate the trade-off between the reconfiguration of SFCs and the optimality of the resulting placement and service flow (re)routing. We model different reconfiguration costs related to the migration of stateful VNFs and solve a joint optimization problem that aims to minimize both the total cost of the VNF placement and the reconfiguration cost necessary for repairing a suboptimal placement. Numerical results show that a small number of reconfiguration operations can significantly reduce the operational cost of the VNF infrastructure; however, too much reconfiguration may not pay off should heavy costs be involved.

==> README <==

March 5, 2007


IEEEtran is the official LaTeX class for authors of the Institute of
Electrical and Electronics Engineers (IEEE) transactions journals and
conferences. The latest version of the IEEEtran package can be found
at CTAN:

http://www.ctan.org/tex-archive/macros/latex/contrib/IEEEtran/

as well as within IEEE's site:

http://www.ieee.org/

For latest news, helpful tips, answers to frequently asked questions,
beta releases and other support, visit the IEEEtran home page at my
website:

http://www.michaelshell.org/tex/ieeetran/


Version 1.7a is a bug fix release that corrects the two column peer
review title page problem. This problem was not present in the 1.6 series.


V1.7 is a significant update over the 1.6 series with many important
changes. For a full list, please read the file changelog.txt. The most
notable changes include:

 1. New class option compsoc to support the IEEE Computer Society format.

 2. Several commands and environments have been deprecated in favor of
    replacements with IEEE prefixes to better avoid potential future name
    clashes with other packages. Legacy code retained to allow the use of
    the obsolete forms (for now), but with a warning message to the console
    during compilation:
    \IEEEauthorblockA, \IEEEauthorblockN, \IEEEauthorrefmark,
    \IEEEbiography, \IEEEbiographynophoto, \IEEEkeywords, \IEEEPARstart,
    \IEEEproof, \IEEEpubid, \IEEEpubidadjcol, \IEEEQED, \IEEEQEDclosed,
    \IEEEQEDopen, \IEEEspecialpapernotice. IEEEtran.cls now redefines
    \proof in way to avoid problems with the amsthm.sty package.
    For IED lists:
    \IEEEiedlabeljustifyc, \IEEEiedlabeljustifyl, \IEEEiedlabeljustifyr,
    \IEEEnocalcleftmargin, \IEEElabelindent, \IEEEsetlabelwidth,
    \IEEEusemathlabelsep
    These commands/lengths now require the IEEE prefix and do not have
    legacy support: \IEEEnormaljot.
    For IED lists: \ifIEEEnocalcleftmargin, \ifIEEEnolabelindentfactor,
    \IEEEiedlistdecl, \IEEElabelindentfactor

 3. New \CLASSINPUT, \CLASSOPTION and \CLASSINFO interface allows for more
    user control and conditional compilation.

 4. Several bug fixes and improved compatibility with other packages.


A note to those who create classes derived from IEEEtran.cls: Consider the
use of patch code, either in an example .tex file or as a .sty file,
rather than creating a new class. The IEEEtran.cls CLASSINPUT interface
allows IEEEtran.cls to be fully programmable with respect to document
margins, so there is no need for new class files just for altered margins.
In this way, authors can benefit from updates to IEEEtran.cls and the need
to maintain derivative classes and backport later IEEEtran.cls revisions
thereto is avoided. As always, developers who create classes derived from
IEEEtran.cls should use a different name for the derived class, so that it
cannot be confused with the official/base version here, as well as provide
authors with technical support for the derived class. It is generally a bad
idea to produce a new class that is not going to be maintained.


Best wishes for all your publication endeavors,

Michael Shell
http://www.michaelshell.org/


********************************** Files **********************************

README                 - This file.

IEEEtran.cls           - The IEEEtran LaTeX class file.

changelog.txt          - The revision history.

IEEEtran_HOWTO.pdf     - The IEEEtran LaTeX class user manual.

bare_conf.tex          - A bare bones starter file for conference papers.

bare_jrnl.tex          - A bare bones starter file for journal papers.

bare_jrnl_compsoc.tex  - A bare bones starter file for Computer Society
                         journal papers.

bare_adv.tex           - A bare bones starter file showing advanced
                         techniques such as conditional compilation,
                         hyperlinks, PDF thumbnails, etc. The illustrated
                         format is for a Computer Society journal paper.

***************************************************************************
Legal Notice:
This code is offered as-is without any warranty either expressed or
implied; without even the implied warranty of MERCHANTABILITY or
FITNESS FOR A PARTICULAR PURPOSE! 
User assumes all risk.
In no event shall IEEE or any contributor to this code be liable for
any damages or losses, including, but not limited to, incidental,
consequential, or any other damages, resulting from the use or misuse
of any information contained here.

All comments are the opinions of their respective authors and are not
necessarily endorsed by the IEEE.

This work is distributed under the LaTeX Project Public License (LPPL)
( http://www.latex-project.org/ ) version 1.3, and may be freely used,
distributed and modified. A copy of the LPPL, version 1.3, is included
in the base LaTeX documentation of all distributions of LaTeX released
2003/12/01 or later.
Retain all contribution notices and credits.
** Modified files should be clearly indicated as such, including  **
** renaming them and changing author support contact information. **

File list of work: IEEEtran.cls, IEEEtran_HOWTO.pdf, bare_adv.tex,
                   bare_conf.tex, bare_jrnl.tex, bare_jrnl_compsoc.tex
***************************************************************************


==> related.tex <==
\subsection{Need for SFC Reconfiguration}
Network providers may need to reconfigure their SFCs for various reasons:

\textbf{Scheduled Migration:} To conduct a set of scheduled actions in a network such as server maintenance, providers might need to migrate VNFs away from a specific server.

\textbf{Change in Objective:} Different placements of VNFs in the network realize different objectives (e.g., energy optimal versus resilient). When objectives change, a reconfiguration might be needed.

\textbf{Consolidation of Suboptimal Placement:} Typically, deployment of new SFCs is done iteratively over time. As requests for the deployment of new SFCs arrive in different time slots, placement algorithms find optimal solutions for VNFs in accordance with available resources in the network for the given time slot. However, as SFCs that have been deployed in previous time slots are typically not changed when new ones are placed, such iterative placement is not globally optimal. Moreover, termination of existing SFCs may lead to fragmentation of resources, which decreases resource utilization of both servers and network. Consequently, optimal placement of a set of SFCs may become suboptimal as time passes, which requires to re-optimize the placement of VNFs using SFC reconfigurations. 

\textbf{Constraints Violation:} Changes in traffic or resource demands may lead to constraint violation. For example, if the optimal placement fully utilizes a set of links or servers, load increase leads to link congestion or CPU contention. In such a scenario, service flow or VNF migration is required. Likewise, in other conditions such as unpredicted link, router, or server failures SFC reconfiguration is required.

\subsection{Reconfiguration Options:} MNOs may have different preferences for managing SFC reconfiguration. For instance, a provider may want to minimize the number of VNF migrations while the other provider is reluctant to relocate VNFs that have a high workload. Even for the same reconfiguration strategy, for example minimizing the number of migrations, MNOs may have different motivations. For instance an MNO may want to minimize the number of migrations for VNFs that have a large memory and disc footprint while the other MNO may desire to minimize VNF migration not because of the size but due to problems such as switch straggler, that flow re-routing may cause in their network~\cite{Gandhi:2017:CUP:3143361.3143397}. 

\subsection{SFC Reconfiguration Operations:} Reconfiguration of SFCs can involve the following set of actions: i) re-routing corresponding service flows served by the VNFs in the network (flow migration), ii) creation, termination, and migration of VNF instances, iii) changing the resource allocation to VNFs.

\textbf{Flow Migration:} Although the problem of flow migration for VNF has not been extensively investigated, it is similar to the traffic reconfiguration problem between network nodes that is addressed in e.g.,~\cite{Gandhi:2017:CUP:3143361.3143397, Hong:2013:AHU:2486001.2486012, Jin:2014:DSN:2619239.2626307, Katta:2013:ICU:2491185.2491191, Liu:2013:ZUD:2486001.2486005, Mahajan:2013:CUS:2535771.2535791, 7497232}. The main objective in these research is to implement consistent routing updates. Such approaches can be extended for VNF flow migration when a problem in the network degrades the performance of SFCs.

\textbf{Creation \& Termination \& Relocation:} VNFs can be categorized into two groups: i) stateless, and ii) stateful. The former types of VNF (e.g., stateless load balancers) either do not store flow states or keep them on a remote data store infrastructure (e.g., using key-value stores) and retrieve them on demand~\cite{Kablan:2015:SNF:2785989.2785993}. Stateful VNFs, on the other hand, maintain flow states locally due to performance concerns or design.

For stateless VNF, reconfiguration costs are mainly due to the overhead on end-hosts and flow migration. Additionally, temporary QoS degradation during the time of VNF creation and termination is another important cost to be considered. In the context of stateful VNFs, VNF reconfiguration is even more costly as VNF state migration is also required, typically involving VM or container migration. VM migration transfers disc, memory and CPU states over the network to the new host and may result in significant stress for hypervisors for serializing (dirty) memory pages and disc contents. 

Authors in~\cite{tajiki} proposed a joint-optimization model for \textit{stateless} VNFs with the objective of minimizing the total power consumption and reconfiguration effort. However, authors only considered the difference in the routing matrix before and after the reconfiguration as the reconfiguration cost, which does not reflect the reconfiguration cost of stateful VNFs. Authors in~\cite{7866881, 7335318} characterized the migration cost by a penalty value, Carpio et al.~\cite{8406275} considered the service disruption due to VNF migration as a cost, Tang~\cite{8338124} modeled the reconfiguration cost by the time that it takes to migrate a VNF instance, and Eramo~\cite{7866881} represented the reconfiguration cost by the revenue loss during the time that the VNF is unable to provide a service due to migration. Although considering the effort required to change the placement of VNFs is crucial, a single parameter as the reconfiguration cost does not represent the complexity and overhead of reconfiguration. In addition, parameters such as duration of migration as well as the migration downtime vary based on the traffic load of the network, and should be modeled more accurately rather than assuming a fixed value as in~\cite{8338124, 7866881}. Finally, to the best of our knowledge the trade-off between optimality and reconfiguration costs in the context of SFCs is not thoroughly investigated before.
